3-D Material Style Transfer for Reconstructing Unknown Appearance in Complex Natural Materials

We propose a 3-D material style transfer framework for reconstructing invisible (or faded) appearance properties in complex natural materials. Our algorithm addresses the technical challenge of transferring appearance properties from one object to another of the same material when both objects have intricate, noncorresponding color patterns. Eggshells, exoskeletons, and minerals, for example, have patterns composed of highly randomized layers of organic and inorganic compounds. These materials pose a challenge as the distribution of compounds that determine surface color changes from object to object and within local pattern regions. Our solution adapts appearance observations from a material property distribution in an exemplar to the material property distribution of a target object to reconstruct its unknown appearance. We use measured reflectance in 3-D bispectral textures to record changing material property distributions. Our novel implementation of spherical harmonics uses principles from chemistry and biology to learn relationships between color (hue and saturation) and material composition and concentration in an exemplar. The encoded relationships are transformed to the property distribution of a target for color recovery and material assignment. Quantitative and qualitative evaluation methods show that we replicate color patterns more accurately than methods that only rely on shape correspondences and coarse-level perceptual differences. We demonstrate applications of our work for reconstructing color in extinct fossils, restoring faded artifacts and generating synthetic textures.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> fig-properties.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\hsize]{images/properties/properties-v002.eps}
\caption{\label{fig:properties}%
Properties for pattern matching. (left to right): color and bispectral reflectance, saturation and bispectral intensity, and curvature. Hue and value properties are transferred for texture generation.}
\end{figure}



==> similar_shape_and_pattern_test.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.4\hsize]{images/results/final_result_cropped.eps}
\caption{\label{fig:final_result}%
Left: Example shell with visible color texture. Right: Target shell with generated color texture.}
\end{figure}



==> texturetransfer.tex <==
1\section{SIMULATING BIO-MATERIALS} \label{simbiomat}
We present an application of our pipeline for the reconstruction of the appearance of fossilized shells for the task of species classification. Our target is the \emph{Conus delesertti} fossil~\ref{fig:uvandsamples}. Figure~\ref{reconstruction} shows the different components of our reconstruction pipeline visualized using different non-photrealistic rendering algorithms. We combine the data acquired and processed in our acquistion and multispectral processing stages to generate a multispectral 3D simulation of the target. Section~\ref{sec:patternextract} describes the mapping of UV patterns to the 3D model of the fossil and Section~\ref{sec:patternmatching} explains our process for pattern matching and texture transfer. In Section~\ref{sec:colorandrefsim} we discuss our strategy for reconstructing the appearance of the fossilized shell. Section~\ref{sec:biolimiations} discusses the limitations of our algorithm and the future direction of this research.


\section{UV Texture Mapping} \label{sec:patternextract}
We capture high resolution UV fluorescence images of the specimen using our UV fluorescence imaging system (Section~\ref{multispectralimaging}). We also capture low resolution UV fluorescence textures along with the 3D model of the specimen using our 3D UV scanning system (Section~\ref{3duvscanning}). We then align the high resolution images to the 3D model in a 3D edting software using UV fluorescent textures as correspondences. Figure~\ref{fig:patternextract} (right) shows the 3D model of the fossil textured with UV fluorescence texture. The color patterns from the texture are used in our pattern matching algorithm for identifying the modern descendant of the fossil and the transfer of colors of the modern shell to the patterns of the fossil.


\section{Pattern Matching and Texture Transfer} \label{sec:patternmatching}
 
We maintain a database of color pattern images, 3D models and primary and secondary specular and diffuse reflectance values of modern shells. Primary refers to the reflectance values measured from the color patterns on the surface of the shells. Secondary reflectance values are measured from regions on the surface without color patterns. Our 3D application~\ref{fig:patternmatch} allows users to select a region of the color patterns from the textured model of the target and match it against color pattern images from the database. Figure~\ref{fig:patternmatch} shows our pattern matching interface. For the current reconstruction task, we asked an expert to assist in matching the target fossil to its closest modern relative in our database (Section~\ref{sec:appuserstudy}).


\paragraph{Background: Conformal mapping} Next, we use conformal mapping~\cite{haker} to map the patterns from the selected modern shell to the patterns of the fossil. Let's recall how conformal mapping works. A conformal mapping is a function that preserves the magnitude and orientation of local angles. Formally, an analytic function $f:U \rightarrow V$, $U, V \in \mathbf{R^{n}}$, is conformal at a point $u_{0} \in U$ if it preserves the magnitude and orientation of angles between the directed curves through $u_{0}$. $f$ has a non-zero derivative at $u_{0}$. 

Conformal mapping is often used to map one genus zero surface (surfaces without any holes or self intersections) to another genus zero surface~\cite{haker, xianfeng, levy}. These algorithms are based on a theory of Riemann surfaces from complex analysis and geometry which states that any genus zero surface can be mapped conformally onto a sphere. Let $\Sigma \in \mathbf{R_{3}}$ be a genus zero smooth model. Let $p$ be a point on the surface of $\Sigma$ and let $\delta_{p}$ denote the Dirac delta (impulse) function at $p$. Let $\mathbf{S^{2}}$ denote a unit sphere in $\mathbf{R^{3}}$ and let $\mathbf{C}$ be a complex plane. A conformal map $z:\Sigma\setminus\{p\}\rightarrow \mathbf{S^{2}\setminus\{north pole\}}$ can be computed by solving the second order partial differential equation given in Equation~\ref{eq:conformalpde} over the surface of $\Sigma$

\begin{equation}
\label{eq:conformalpde}
\Delta z = \left(  \frac{\partial}{\partial u} - \iota \frac{\partial}{\partial v} \right) \delta_{p}
\end{equation}

where $u$ and $v$ are conformal coordinates defined in neighborhood of $p$, $\iota$ is the square root of $-1$ and $\Delta$ is the Laplace-Beltrami operator, a generalization of the Laplace operator to a smooth surface. Conformal coordinates $u$,$v$ are chosen such that the metric at $p$ is of the form $ds^{2} = \lambda( u, v )^{2} ( du^{2} + dv^{2} )$ with an initial value $u = v = 0$ which maps $p$ to the north pole of $\mathbf{S^{2}}$. Equation~\ref{eq:conformalpde} assumes $\Sigma$ is a smooth manifold with smooth functions. To solve for triangulated surfaces, the functions on the simplicial complex of $\Sigma$ are approximated as piecewise linear functions. Simplicial complex of a triangulated mesh is the set of points, line segments, triangles and other n-dimensional simplicies that comprise the mesh. Next, equation~\ref{eq:conformalpde} is solved for each surface point $q \in \Sigma\setminus\{p\}$ to generate a vector of complex numbers $\mathbf{h}$ that map each $q$ to a point $(u, v)$ in $\mathbf{C}$. Finally, to map $(u, v)$ to a point $(X, Y, Z)$ on $\mathbf{S^{2}}$, an inverse stereo-projection is used as given in Equations~\ref{eq:invstereox},~\ref{eq:invstereoy} and~\ref{eq:invstereoz}

\begin{equation}
	\label{eq:invstereox}
	X = \left( \frac{2u}{1 + r^{2}} \right)
\end{equation}

\begin{equation}
\label{eq:invstereoy}
	Y = \left( \frac{2v}{1 + r^{2}} \right)
\end{equation}

\begin{equation}
\label{eq:invstereoz}
	Z = \left( \frac{2r^{2}}{1 + r^{2} - 1} \right)
\end{equation}

where $r^{2} = u^{2} + v^{2}$.

The conformal mapping of a Riemannian manifold to a sphere is unique only upto a scaling and translation factor. The space of all such transformations that conformally map a manifold to a sphere are called Mobius transformations. To generate a unique mapping $\phi$ between two genus zero surfaces $M$ and $N$ mapped to the same unit sphere, an iterative energy minimization technique is used that minimizes the harmonic energy of $\phi$. Harmonic energy is the energy of the mapping $\phi$ between $M$ and $N$ and is given by Equation~\ref{eq:harmonicenergy}

\begin{equation}
\label{eq:harmonicenergy}
E(\phi) = \int_{M} \|du\|^{2} d\mu_{M}
\end{equation}   

where the norm of the differential $\|du\|$ is computed from a metric on $M$ and $N$ and $d\mu_{M}$ is the measure on $M$. At each iteration, first the vector of derivatives $D\mathbf{h}$ of $\mathbf{h}$ is computed and is used to update $\mathbf{h}$. Then, a new mobius transformation is computed that minmizes the metric on $M$ and $N$. Finally harmonic energy $E$ is computed for the new transformation and compared against a threshold $E_{0}$. The process is repeated untill $E < E_{0}$. The above conformal mapping process only compares the overall shape of the two 3D models. Additional constraints are required to map individual geometric features of the two surfaces.

%For brain surface mapping~\ref{} an additional optimization step is used that adjusts the conformal parameterization to match the geometric featues of the brain. In preprocessing step, landmarks, in form curves, are drawn over the two surfaces $M$ and $N$ and correspondence between the curves are assigned. Then, in the optimization step, matching energy is computed and iteratively minimized by minmizing the Eculidean distance between the corresponding curves on the two surfaces. 

Our goal is to recover the correct color information from the texture of a modern shell to color the patterns of the fossil. There are several technical challenges with this problem. The correspondence between the color patterns between the two shells is unknown apriori. The shape of the patterns also vary widely from shell to shell. Finally, there are variations in color within a single pattern which need to be captured for accurate appearance reconstruction. Existing techniques are unsuitable for this task because they only consider the variations in local shape for generating a mapping between the two surfaces. We present an algorithm that uses conformal mapping and energy minimzation techniques to find the correspondences between patterns of the two shells and transfers both the color and the variations in color with in each pattern, from modern shell to the fossil. Figure~\ref{fig:texturetransfer} shows the intermediate results of our algorithm.


First, we conformally map the surfaces of the fossilized shell $S_{1}$ and the modern shell $S_{2}$ to a sphere $\mathbf{S^{2}}$ using the technique described above. We compute spherical co-ordinates for each point on the sphere and use them as texture coordinates to map the textures to the sphere~\cite{haker}. Next, for each surface, we identify points on the sphere that lie on the color patterns to generate patches and match each patch on the fossil to a patch in the modern based on a similarity metric. Our matching algorithm considers the geodesic area and shape of the patches, the variations in the underlying curvatures and the geodesic distance between the modern and fossil patches in the sphere space to compute similarity. For each matched pair, we apply a rigid body transformation to align the centers of the patches and locally orient the modern patch to the coordinate frame of the fossil patch. Then, we sample vertices on the modern patch, transfer the color and gradient properties of the texture to the corresponding points on the fossil, and use a heat diffusion algorithm to propagate these properties to the vertices of the fossil. Finally, we apply an inverse conformal transformation to the fossil mesh to recover the original shape of the fossil. 

\section{Appearance Reconstruction} \label{sec:colorandrefsim}
The inputs to our appearance reconstruction algorithm are: a 3D model of the fossil, UV fluorescence texture $T_{v}$, recovered texture $T_{f}$, and sets of primary and secondary diffuse and specular reflectance values, $D_{p}$, $S_{p}$, $D_{s}$ and $S_{s}$, of the modern shell. We apply Blinn-Phong shading (Equation~\ref{equ:blinnphong}) to the model to simulate the diffuse and specular reflectance characteristics of the shell. At each surface point $p$, we first verify whether $p$ lies on a pattern using $T_{v}$ and sample the diffuse and specular reflectance values from the appropriate reflectance dataset (primary or secondary). Next, we sample the color from $T_{f}$ and scale it with the reflectance values to compute $k_{d}$ and $k_{s}$. We substitue these values in Equation~\ref{equ:blinnphong} to generate the final color. 



   


        




         

